The $S$-diagnostic -- an a posteriori error assessment for single-reference coupled-cluster methods

We propose a novel a posteriori error assessment for the single-reference coupled-cluster (SRCC) method called the $S$-diagnostic. We provide a derivation of the $S$-diagnostic that is rooted in the mathematical analysis of different SRCC variants. We numerically scrutinized the $S$-diagnostic, testing its performance for (1) geometry optimizations, (2) electronic correlation simulations of systems with varying numerical difficulty, and (3) the square-planar copper complexes [CuCl$_4$]$^{2-}$, [Cu(NH$_3$)$_4$]$^{2+}$, and [Cu(H$_2$O)$_4$]$^{2+}$. Throughout the numerical investigations, the $S$-diagnostic is compared to other SRCC diagnostic procedures, that is, the $T_1$, $D_1$, and $D_2$ diagnostics as well as different indices of multi-determinantal and multi-reference character in coupled-cluster theory. Our numerical investigations show that the $S$-diagnostic outperforms the $T_1$, $D_1$, and $D_2$ diagnostics and is comparable to the indices of multi-determinantal and multi-reference character in coupled-cluster theory in their individual fields of applicability. The experiments investigating the performance of the $S$-diagnostic for geometry optimizations using SRCC reveal that the $S$-diagnostic correlates well with different error measures at a high level of statistical relevance. The experiments investigating the performance of the $S$-diagnostic for electronic correlation simulations show that the $S$-diagnostic correctly predicts strong multi-reference regimes. The $S$-diagnostic moreover correctly detects the successful SRCC computations for [CuCl$_4$]$^{2-}$, [Cu(NH$_3$)$_4$]$^{2+}$, and [Cu(H$_2$O)$_4$]$^{2+}$, which have been known to be misdiagnosed by $T_1$ and $D_1$ diagnostics in the past. This shows that the $S$-diagnostic is a promising candidate for an a posteriori diagnostic for SRCC calculations.

==> CC diagnostics-w-bbl/table.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
Molecule
&
T1
&
D1
&
D2
&
S1
&
S2
&
S3
&
r$_e$ (Exp)
&
r$_e$ (CC)
&
r$_e$ (Diff)
\\
\hline
$CH_2$
&
0.004
&
0.008
&
0.416
&
1.248
&
2.31
&
2.058
&
$\begin{bmatrix}
  -1. & 1.0775 & 1.0775\\
  1.0775 & -1. & 2.155\\
  1.0775 & 2.155 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.085 & 1.085\\
  1.085 & -1. & 2.0084\\
  1.085 & 2.0084 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0075 & 0.0075\\
  0.0075 & 0. & 0.1466\\
  0.0075 & 0.1466 & 0.\\
\end{bmatrix}$
\\
$H_2N_2$
&
0.01
&
0.032
&
0.202
&
0.362
&
0.705
&
0.683
&
$\begin{bmatrix}
  -1. & 1.2549 & 1.0415 & 1.8308\\
  1.2549 & -1. & 1.8308 & 1.0415\\
  1.0415 & 1.8308 & -1. & 2.7015\\
  1.8308 & 1.0415 & 2.7015 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.252 & 1.028 & 1.8294\\
  1.252 & -1. & 1.8294 & 1.028\\
  1.028 & 1.8294 & -1. & 2.6906\\
  1.8294 & 1.028 & 2.6906 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0029 & 0.0135 & 0.0014\\
  0.0029 & 0. & 0.0014 & 0.0135\\
  0.0135 & 0.0014 & 0. & 0.0109\\
  0.0014 & 0.0135 & 0.0109 & 0.\\
\end{bmatrix}$
\\
$HOF$
&
0.01
&
0.037
&
0.197
&
0.27
&
0.526
&
0.511
&
$\begin{bmatrix}
  -1. & 0.9725 & 1.4416\\
  0.9725 & -1. & 1.8403\\
  1.4416 & 1.8403 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 0.96 & 1.442\\
  0.96 & -1. & 1.8297\\
  1.442 & 1.8297 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0125 & 0.0004\\
  0.0125 & 0. & 0.0106\\
  0.0004 & 0.0106 & 0.\\
\end{bmatrix}$
\\
$C_2H_2$
&
0.011
&
0.027
&
0.184
&
0.295
&
0.578
&
0.563
&
$\begin{bmatrix}
  -1. & 1.2219 & 1.077 & 2.2989\\
  1.2219 & -1. & 2.2989 & 1.077\\
  1.077 & 2.2989 & -1. & 3.3758\\
  2.2989 & 1.077 & 3.3758 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.2026 & 1.0631 & 2.2657\\
  1.2026 & -1. & 2.2657 & 1.0631\\
  1.0631 & 2.2657 & -1. & 3.3288\\
  2.2657 & 1.0631 & 3.3288 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0193 & 0.0139 & 0.0332\\
  0.0193 & 0. & 0.0332 & 0.0139\\
  0.0139 & 0.0332 & 0. & 0.047\\
  0.0332 & 0.0139 & 0.047 & 0.\\
\end{bmatrix}$
\\
$ClOH$
&
0.007
&
0.024
&
0.182
&
0.317
&
0.62
&
0.604
&
$\begin{bmatrix}
  -1. & 0.9707 & 1.7353\\
  0.9707 & -1. & 2.1471\\
  1.7353 & 2.1471 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 0.9732 & 1.6974\\
  0.9732 & -1. & 2.1309\\
  1.6974 & 2.1309 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0025 & 0.0379\\
  0.0025 & 0. & 0.0162\\
  0.0379 & 0.0162 & 0.\\
\end{bmatrix}$
\\
\end{tabular}


==> table.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
Molecule
&
T1
&
D1
&
D2
&
S1
&
S2
&
S3
&
r$_e$ (Exp)
&
r$_e$ (CC)
&
r$_e$ (Diff)
\\
\hline
$CH_2$
&
0.004
&
0.008
&
0.416
&
1.248
&
2.31
&
2.058
&
$\begin{bmatrix}
  -1. & 1.0775 & 1.0775\\
  1.0775 & -1. & 2.155\\
  1.0775 & 2.155 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.085 & 1.085\\
  1.085 & -1. & 2.0084\\
  1.085 & 2.0084 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0075 & 0.0075\\
  0.0075 & 0. & 0.1466\\
  0.0075 & 0.1466 & 0.\\
\end{bmatrix}$
\\
$H_2N_2$
&
0.01
&
0.032
&
0.202
&
0.362
&
0.705
&
0.683
&
$\begin{bmatrix}
  -1. & 1.2549 & 1.0415 & 1.8308\\
  1.2549 & -1. & 1.8308 & 1.0415\\
  1.0415 & 1.8308 & -1. & 2.7015\\
  1.8308 & 1.0415 & 2.7015 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.252 & 1.028 & 1.8294\\
  1.252 & -1. & 1.8294 & 1.028\\
  1.028 & 1.8294 & -1. & 2.6906\\
  1.8294 & 1.028 & 2.6906 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0029 & 0.0135 & 0.0014\\
  0.0029 & 0. & 0.0014 & 0.0135\\
  0.0135 & 0.0014 & 0. & 0.0109\\
  0.0014 & 0.0135 & 0.0109 & 0.\\
\end{bmatrix}$
\\
$HOF$
&
0.01
&
0.037
&
0.197
&
0.27
&
0.526
&
0.511
&
$\begin{bmatrix}
  -1. & 0.9725 & 1.4416\\
  0.9725 & -1. & 1.8403\\
  1.4416 & 1.8403 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 0.96 & 1.442\\
  0.96 & -1. & 1.8297\\
  1.442 & 1.8297 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0125 & 0.0004\\
  0.0125 & 0. & 0.0106\\
  0.0004 & 0.0106 & 0.\\
\end{bmatrix}$
\\
$C_2H_2$
&
0.011
&
0.027
&
0.184
&
0.295
&
0.578
&
0.563
&
$\begin{bmatrix}
  -1. & 1.2219 & 1.077 & 2.2989\\
  1.2219 & -1. & 2.2989 & 1.077\\
  1.077 & 2.2989 & -1. & 3.3758\\
  2.2989 & 1.077 & 3.3758 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 1.2026 & 1.0631 & 2.2657\\
  1.2026 & -1. & 2.2657 & 1.0631\\
  1.0631 & 2.2657 & -1. & 3.3288\\
  2.2657 & 1.0631 & 3.3288 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0193 & 0.0139 & 0.0332\\
  0.0193 & 0. & 0.0332 & 0.0139\\
  0.0139 & 0.0332 & 0. & 0.047\\
  0.0332 & 0.0139 & 0.047 & 0.\\
\end{bmatrix}$
\\
$ClOH$
&
0.007
&
0.024
&
0.182
&
0.317
&
0.62
&
0.604
&
$\begin{bmatrix}
  -1. & 0.9707 & 1.7353\\
  0.9707 & -1. & 2.1471\\
  1.7353 & 2.1471 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  -1. & 0.9732 & 1.6974\\
  0.9732 & -1. & 2.1309\\
  1.6974 & 2.1309 & -1.\\
\end{bmatrix}$
&
$\begin{bmatrix}
  0. & 0.0025 & 0.0379\\
  0.0025 & 0. & 0.0162\\
  0.0379 & 0.0162 & 0.\\
\end{bmatrix}$
\\
\end{tabular}

